Model-Based Insights on the Performance, Fairness, and Stability of BBR

Google's BBR is the most prominent result of the recently revived quest for efficient, fair, and flexible congestion-control algorithms (CCAs). While the performance of BBR has been investigated by numerous studies, previous work still leaves gaps in the understanding of BBR performance: Experiment-based studies generally only consider network settings that researchers can set up with manageable effort, and model-based studies neglect important issues like convergence. To complement previous BBR analyses, this paper presents a fluid model of BBRv1 and BBRv2, allowing both efficient simulation under a wide variety of network settings and analytical treatment such as stability analysis. By experimental validation, we show that our fluid model provides highly accurate predictions of BBR behavior. Through extensive simulations and theoretical analysis, we arrive at several insights into both BBR versions, including a previously unknown bufferbloat issue in BBRv2.

==> sections/motivation.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Why Reconsider Fluid Models?}

Fluid models are one of the most classic
analytical approaches in research on
CCAs.
The central feature of fluid models is the
representation of traffic flows as fluid
streams, i.e., quantities that are continuously
evolving and arbitrarily divisible,
in contrast to discrete sequences of individual
packets. This approximation of
flows allows to describe the network behavior
with ordinary differential 
equations~(ODEs), which in turn contain
continuously differentiable functions
and are thus suitable for analytical
examination. 

Since fluid models do not contain a 
notion of individual packets, they are typically considered to be applicable mainly to 
large-scale networks, where the packet size 
becomes negligible compared to the
overall traffic volumes. Moreover, 
the smooth curves produced by fluid
models arguably describe an ``average'' state of the network
rather than actual traces containing low-level
fluctuations. As a result, fluid models
have mainly been applied to investigate
`systemic' properties of CCAs, e.g.,
control-theoretic 
stability~\cite{srikant2004mathematics,low2002internet,vardoyan2018towards}.
However, while fluid models experienced a surge
of interest in this context around 20
years ago, their popularity has diminished relative to
the increasingly experiment-based
CC research literature ever since. 
% (except for a short-lived revival when
% the stability of multi-path congestion-control
% algorithms became a focus~\cite{peng2013multipath}).

An attractive feature of fluid models is that they do not only
allow to analytically evaluate
stability aspects, but also to
perform numerical computations 
(e.g., using Runge--Kutta methods), as also pioneered around 20 years ago~\cite{misra2000fluid,liu2003fluid}.
Fluid models hence constitute a valuable complement to experimental
evaluations of CCAs, as such numerical computations can compensate
methodological weaknesses of experiments in the following
fields:

\begin{description}[leftmargin = *,topsep=6pt]
\item[Design] Fluid models are created and adjusted more
    easily than full-fledged CCA implementations, as the fluid models 
    can ignore practical concerns such as retransmissions, 
    OS interactions, and software-development issues. 
    Hence, fluid models are ideal 
    for rapid initial analyses and insights.
    
\item[Evaluation set-up] The network model can be adjusted easily 
    for different topologies, including link capacities and delays,
    and router behavior, such as queuing disciplines.
    Moreover, CCA parameters can be varied more easily in
    fluid models. As a result, the evaluation quickly achieves
    systematic and generalizable results.
    
\item[Evaluation execution] Model-based computations are 
    less expensive to conduct than ex\-peri\-ments:
    The computational effort of fluid models is scale-invariant
    to network capacities (different numbers in the same computations), 
    whereas the computational, memory-related
    and monetary cost of experiments generally rises with the tested
    traffic volumes.
    
\item[Evaluation analysis] The identification and
    elimination of bugs and artifacts in model computations is simpler than in experiments,
    for two reasons. First, the source of issues is easier
    to spot in a handful of equations than in
    a program potentially spanning thousands of lines of code.
    Second, model computations can be more thoroughly isolated
    from environmental distortions than experiment executions:
    Network emulators such as mininet~\cite{lantz2010network}
    suffer from persistent glitches, 
    lab experiments are affected by the concrete systems
    of the used machines, and real-world experiments 
    in a production setting are by definition
    influenced by the surrounding network. 
    Finally, the deterministic nature
    of fluid models ensures reproducibility
    of interesting phenomena.
\end{description}

Moreover, various contemporary trends make fluid models an increasingly 
important and viable tool. In particular, network settings
are becoming more diverse and 
the volume of relevant parameter configurations thus grows; as fluid models can save considerable effort
in evaluation set-up, their value thus increases. 
Furthermore, the increasing computational
power and effectiveness of differential-equation solvers make fluid-model computations even faster,
enlarging their advantages in the evaluation
execution. 
Of course, the
methodological strengths of fluid models need to be
set in relation to their predictive accuracy,
which we assess in this paper.

==> sections/numerical-analysis.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical Dependency Analysis}
\label{sec:results}

In this section, we investigate a wide variety
of network configurations by means of the fluid
model that has been presented in~\cref{sec:models}
and validated in~\cref{sec:experiments}.
In contrast to~\cref{sec:experiments},
this section analyzes the performance of
various CCAs on a high-capacity bottleneck 
link as it appears in real network settings:
While we still use the topology from~\cref{fig:topology},
we set a bottleneck-link capacity~$\lcap{}$ of 1 Gbps.
The easiness of this adjustment highlights
a strength of fluid models: Testing
high link capacities is virtually unrestricted
and cost-free in fluid models,
whereas in experiments, more powerful and expensive
hardware is required.

In our analysis, we use the same
numerical approach as in the previous section.
In the setup, we vary the following parameters:
The number of senders~$N$ is varied between 2, 6 and 10,
the bottleneck-link delay~$\propd{}$ is varied between 2.5, 7.5 and \SI{12.5}{\ms},
and the bottleneck-link buffer size~$\lbuf{}$ is varied
between 0.5 and 7 BDP. The delay of the
non-shared links is randomly chosen between 5 and \SI{10}{\ms}
such that RTT ranges of 5--\SI{15}{\ms}, 15--\SI{25}{\ms} and 25--\SI{35}{\ms}
result for the tested bottleneck-link delays.
\cref{fig:results:buffer:droptail,,fig:results:latency:droptail,,fig:results:senders:droptail}
highlight the dependency of various network metrics
(aggregated over 20-second traces)
on buffer size~$\lbuf{}$, latency~$\propd{}$ and
sender count~$N$, respectively, under drop-tail. 
The same dependencies under
RED are shown in~\cref{fig:results:buffer:red,,fig:results:latency:red,,fig:results:senders:red}
We discuss the results in the following subsections.

\begin{figure*}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/B_fairness_cc_combination_droptail.pdf}
        \caption{Fairness}
        \label{fig:results:buffer:droptail:fairness}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/B_loss_cc_combination_droptail.pdf}
        \caption{Loss}
        \label{fig:results:buffer:droptail:loss}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/B_queueing_cc_combination_droptail.pdf}
        \caption{Queuing}
        \label{fig:results:buffer:droptail:queuing}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/B_utilization_cc_combination_droptail.pdf}
        \caption{Utilization}
        \label{fig:results:buffer:droptail:utilization}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Aggregate metric results as buffer-size dependency ($N =\num{10}$ senders, $d_\ell =\SI{7.5}{\ms}$, drop-tail)}
    \label{fig:results:buffer:droptail}
\end{figure*}

\begin{figure*}
    %\vspace{-10pt}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/Lat_fairness_cc_combination_droptail.pdf}
        \caption{Fairness}
        \label{fig:results:latency:droptail:fairness}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/Lat_loss_cc_combination_droptail.pdf}
        \caption{Loss}
        \label{fig:results:latency:droptail:loss}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/Lat_queueing_cc_combination_droptail.pdf}
        \caption{Queuing}
        \label{fig:results:latency:droptail:queuing}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/Lat_utilization_cc_combination_droptail.pdf}
        \caption{Utilization}
        \label{fig:results:latency:droptail:utilization}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Aggregate metric results as link-latency dependency ($N =\num{10}$ senders, $B_\ell =\text{BDP}$, drop-tail)}
    \label{fig:results:latency:droptail}
\end{figure*}



\begin{figure*}
    %\vspace{-10pt}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/N_fairness_cc_combination_droptail.pdf}
        \caption{Fairness}
        \label{fig:results:senders:droptail:fairness}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/N_loss_cc_combination_droptail.pdf}
        \caption{Loss}
        \label{fig:results:senders:droptail:loss}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/N_queueing_cc_combination_droptail.pdf}
        \caption{Queuing}
        \label{fig:results:senders:droptail:queuing}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/N_utilization_cc_combination_droptail.pdf}
        \caption{Utilization}
        \label{fig:results:senders:droptail:utilization}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Aggregate metric results as sender-count dependency ($d_{\ell} =\SI{7.5}{\ms}$, $B_\ell =\text{BDP}$, drop-tail)}
    \label{fig:results:senders:droptail}
\end{figure*}


\subsection{Dependency on Buffer Size}
\label{sec:results:buffer}

In \cref{fig:results:buffer:droptail} 
and~\cref{fig:results:buffer:red}, 
the network metrics fairness, loss, queue size and
utilization are shown in dependence of bottleneck-link
buffer size, as in~\cref{sec:experiments:aggregate}.
Since the results are largely similar
to the model and experiment results in~\cref{sec:experiments:aggregate},
we only discuss deviations here.

First, the unfairness of BBRv1 is even more extreme than
found previously, both in a homogeneous setting
and towards loss-sensitive CCAs in shallow drop-tail buffers.
This unfairness results from differences in estimated BDP
due to different RTTs.
These differences are even larger given the higher-capacity
link in the numerical analysis.

Second, BBRv2 is much more unfair towards the
loss-based CCAs Reno and CUBIC under RED 
for the 1 Gbps links
(cf.~\cref{fig:results:buffer:red:fairness}) 
than for the 100 Mbps link. This additional
unfairness stems from the fact the the loss-based
CCAs recover slowly when operating with
large congestion windows, as necessary on high-capacity
links. For one, Reno cuts the congestion-window size
from ~$w$ to~$w/2$ in case of loss, and therefore requires~$w/2$ RTTs
to restore the window size at the time of loss
because the window grows by 1 segment per RTT
independently of~$w$. Clearly, the loss-recovery
time of Reno thus grows with~$w$. The loss-recovery
time~$s^{\ast}$ of CUBIC as a function of the
congestion-window size is even dominated by 
a cubic term
of~$w$:
\begin{equation}
    s^{\ast}(w) = \Big(\frac{w\cdot c}{b}\Big)^3 -\sqrt[3]{\frac{w}{c}} + 
\end{equation} where~$c$ and~$b$ are the CUBIC
parameters as used in~\cref{eq:w:cubic}.
Hence, the loss sensitivity of Reno and CUBIC
grows with increasing bottleneck-link size,
whereas the loss sensitivity of BBRv2
remains constant. As a result, BBRv2
flows are able to obtain an unfairly high
bandwidth share under RED when competing
with flows employing loss-based CCAs.
Since loss events are less frequent
in drop-tail buffers, the same effect
is not equally powerful in absence
of a RED queuing policy.


\subsection{Dependency on Link Latency}
\label{sec:results:latency}

\cref{fig:results:latency:droptail,,fig:results:latency:red}
illustrate how the latency of the bottleneck link affects
CCA performance under drop-tail and RED, respectively.


Regarding fairness 
(\cref{fig:results:latency:droptail:fairness,,fig:results:latency:red:fairness}),
BBRv1's unfairness towards Reno and CUBIC
appears to be independent of link latency,
whereas the fairness of BBRv1 in a homogeneous
setting and the fairness of loss-sensitive CCAs in both
homogeneous and heterogeneous settings
is increasing together with RTT.
Two factors drive this positive relationship
of bottleneck-link delay with fairness.
First, due to our fixed choice
of 10-millisecond RTT ranges, the \emph{relative}
latency differences between flows diminish
for increasing bottleneck-link delays.
Hence, CCAs that suffer from RTT unfairness
(BBRv1, BBRv2 and Reno) have a less skewed
distribution of obtained bandwidth shares
across flows.
Second, since the buffer size equals 1 BDP
of the bottleneck link, longer bottleneck-link
delays are associated with larger buffers.
These larger buffers lead to fewer loss events,
which allows Reno and CUBIC to compete more effectively
against BBRv2 and thus leads to improved
fairness for this combination.

Regarding loss, the bottleneck-link latency has no effect 
in drop-tail buffers that would be discernible 
in~\cref{fig:results:latency:droptail:loss}.
For RED, however, loss is decreasing as a function
of RTT for CCA combinations involving BBRv1 
(\cref{fig:results:latency:red:loss}).
This decrease in loss can be explained
by the reduced relative buffer utilization
of BBRv1, which determines the loss
rate in a RED queuing discipline.
The reduced buffer utilization itself is 
the result of the absolute buffering volume
of BBRv1 remaining constant while
buffers become larger due to the
previously mentioned dependence of
buffer size on bottleneck-link delay.

Queueing in drop-tail buffers (\cref{fig:results:buffer:droptail:queuing}) 
exhibits bufferbloat for all combinations involving
BBRv1. The delay dependence of BBRv2 is nonlinear
because (1) BBRv2 leads to a constant absolute queuing
volume, which appears as reduced buffer utilization
for growing buffers, and (2) BBRv2 is loss-sensitive,
which reduces its buffer utilization in small buffers
(e.g., for a delay of 2.5 ms) that cause frequent loss
events. The buffer occupancy of CUBIC is equally
non-linear because small buffers increase
the frequency of loss events, but large buffers
force CUBIC to operate with larger congestion windows,
which recover more slowly from loss than smaller windows.
In contrast, the delay dependence of Reno is linearly
negative, because the loss-recovery time of Reno
does not only depend on the congestion-window size
at the time of loss, but in addition on the RTT.
Hence, the low RTT of 2.5 milliseconds outweighs
the more frequent loss events in the smaller
buffer in that scenario.

Regarding utilization, all CCA combinations utilize
the bottleneck link almost completely given a drop-tail
queuing discipline (cf. y-axis in~\cref{fig:results:buffer:droptail:utilization}).
For a RED queuing discipline, however, the utilization
achieved by loss-sensitive CCAs is incomplete
(cf.~\cref{fig:results:buffer:red:utilization}),
because loss-sensitive CCAs
reduce their rate when the buffer even starts filling up
and the RED algorithm starts to drop packets.
The non-linear dependence of bottleneck-link delay
on the utilization by the BBRv2/Reno combination
is driven by the combined effects of more frequent
loss events given shorter RTTs and faster loss recovery
given shorter RTTs, which make the aggregate effect
on utilization ambivalent.

\subsection{Dependency on Sender Count}
\label{sec:results:senders}

Finally, we discuss the effects of the number of senders
on CCA performance, as visualized 
in~\cref{fig:results:senders:droptail,,fig:results:senders:red}.

Regarding fairness, the number of senders has
no effects on CCA combinations that are
either completely fair (BBRv1 and BBRv2)
in homogeneous settings or completely
unfair (BBRv1 combined with Reno or CUBIC,
respectively). As an exception, a BBRv2 flow
can uphold a non-negligible sending rate 
in the face of a single BBRv1 flow,
but not for higher numbers of competing
BBRv1 flows. The fairness of combinations
of loss-sensitive CCAs has a modestly
positive relationship with the number of
senders, which can be explained by the higher
variance in smaller sender populations.

Unsurprisingly, the remaining metrics loss, 
queuing and utilization are positively affected
by the number of senders, simply because
multiple flows are more aggressive
than a single flow for any CCA.
Interestingly, the only scenario
in which BBRv1 does not achieve full
buffer utilization is when one BBRv1 flow
competes with one flow employing a
loss-sensitive CCA, i.e., for two senders
in total. This insight confirms the high
aggressiveness of BBRv1.

\begin{figure*}[!h]
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/B_fairness_cc_combination_RED.pdf}
        \caption{Fairness}
        \label{fig:results:buffer:red:fairness}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/B_loss_cc_combination_RED.pdf}
        \caption{Loss}
        \label{fig:results:buffer:red:loss}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/B_queueing_cc_combination_RED.pdf}
        \caption{Queuing}
        \label{fig:results:buffer:red:queuing}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/B_utilization_cc_combination_RED.pdf}
        \caption{Utilization}
        \label{fig:results:buffer:red:utilization}
    \end{subfigure}
    \vspace{-10pt}
    \caption{Aggregate metric results as buffer-size dependency ($N =\num{10}$ senders, $d_\ell =\SI{7.5}{\ms}$, RED)}
    \label{fig:results:buffer:red}
    \vspace{-10pt}
\end{figure*}

\begin{figure*}[!h]
    %\vspace{-10pt}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/Lat_fairness_cc_combination_RED.pdf}
        \caption{Fairness}
        \label{fig:results:latency:red:fairness}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/Lat_loss_cc_combination_RED.pdf}
        \caption{Loss}
        \label{fig:results:latency:red:loss}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/Lat_queueing_cc_combination_RED.pdf}
        \caption{Queuing}
        \label{fig:results:latency:red:queuing}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/Lat_utilization_cc_combination_RED.pdf}
        \caption{Utilization}
        \label{fig:results:latency:red:utilization}
    \end{subfigure}
    \caption{Aggregate metric results as link-latency dependency ($N =\num{10}$ senders, $B_\ell =\text{BDP}$, RED)}
    \label{fig:results:latency:red}
\end{figure*}


\begin{figure*}[!h]
    %\vspace{-10pt}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/N_fairness_cc_combination_RED.pdf}
        \caption{Fairness}
        \label{fig:results:senders:red:fairness}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/N_loss_cc_combination_RED.pdf}
        \caption{Loss}
        \label{fig:results:senders:red:loss}
    \end{subfigure}
    \begin{subfigure}[b]{0.2\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/N_queueing_cc_combination_RED.pdf}
        \caption{Queuing}
        \label{fig:results:senders:red:queuing}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/results/aggregate/N_utilization_cc_combination_RED.pdf}
        \caption{Utilization}
        \label{fig:results:senders:red:utilization}
    \end{subfigure}
    \caption{Aggregate metric results as population dependency ($d_{\ell} =\SI{7.5}{\ms}$, $B_\ell =\text{BDP}$, RED)}
    \label{fig:results:senders:red}
\end{figure*}
